IR-Aware ECO Timing Optimization Using Reinforcement Learning

Engineering change orders (ECOs) in late stages make minimal design fixes to recover from timing shifts due to excessive IR drops. This paper integrates IR-drop-aware timing analysis and ECO timing optimization using reinforcement learning (RL). The method operates after physical design and power grid synthesis, and rectifies IR-drop-induced timing degradation through gate sizing. It incorporates the Lagrangian relaxation (LR) technique into a novel RL framework, which trains a relational graph convolutional network (R-GCN) agent to sequentially size gates to fix timing violations. The R-GCN agent outperforms a classical LR-only algorithm: in an open 45nm technology, it (a) moves the Pareto front of the delay-power tradeoff curve to the left (b) saves runtime over the prior approaches by running fast inference using trained models, and (c) reduces the perturbation to placement by sizing fewer cells. The RL model is transferable across timing specifications and to unseen designs with fine tuning.

==> misc/bibfile <==
@string{cad = "IEEE Transactions on Computer-Aided Design of Integrated
	Circuits and Systems"}
@string{comp = "IEEE Transactions on Computers"}
@string{cas = "IEEE Transactions on Circuits and Systems"}
@string{cas1 = "IEEE Transactions on Circuits and Systems I"}
@string{cas2 = "IEEE Transactions on Circuits and Systems II"}
@string{ibm = "IBM Journal of Research and Development"}
@string{ed = "IEEE Transactions on Electron Devices"}
@string{edl = "IEEE Electron Device Letters"}
@string{tvlsi = "IEEE Transactions on VLSI Systems"}
@string{cpmt = "IEEE Transactions on Components and Packaging Technologies"}
@string{tdmr = "IEEE Transactions on Devices and Materials Reliability"}
@string{solid = "IEEE Journal of Solid-State Circuits"}
@string{tc = "IEEE Transactions on Computers"}
@string{iccadold = "Proceedings of the IEEE International Conference on
	Computer-Aided Design"}
@string{iccad = "Proceedings of the IEEE/ACM International Conference on
	Computer-Aided Design"}
@string{dac = "Proceedings of the ACM/IEEE Design Automation Conference"}
@string{dacnew = "Proceedings of the ACM/EDAC/IEEE Design Automation Conference"}
@string{dacnewnew = "Proceedings of the ACM/ESDA/IEEE Design Automation Conference"}
@string{aspdac = "Proceedings of the Asia-South Pacific Design Automation
	Conference"}
@string{edac = "Proceedings of the European Design Automation Conference"}
@string{dateconf = "Proceedings of Design, Automation \& Test in Europe"}
@string{iscas = "Proceedings of the IEEE International Symposium on Circuits
	and Systems"}
@string{itc = "Proceedings of the IEEE International Test Conference"}
@string{iccd = "Proceedings of the IEEE International Conference on Computer
	Design"}
@string{cicc = "Proceedings of the IEEE Custom Integrated Circuits Conference"}
@string{ieeepr = "Proceedings of the IEEE"}
@string{mnr = "Microelectronics and Reliability"}
@string{isscc = "Proceedings of the IEEE International Solid-State Circuits
	Conference"}
@string{hotchips = "Proceedings of the IEEE HotChips Symposium"}
@string{isqed = "Proceedings of the IEEE International Symposium on Quality
	Electronic Design"}
@string{edl = "IEEE Electron Device Letters"}
@string{ispd = "Proceedings of the International Symposium on Physical Design"}
@string{dnt = "IEEE Design \& Test"}
@string{islped = "Proceedings of the ACM International Symposium on Low Power
	Electronics and Design"}
@string{iedm = "IEEE International Electronic Devices Meeting"}
@string{irps = "Proceedings of the IEEE International Reliability Physics
	Symposium"}
@string{isca = "Proceedings of the ACM International Symposium on Computer
	Architecture"}
@string{todaes = "ACM Transactions on Design Automation of
	Electronic Systems"}
@string{irps = "IEEE International Reliability Physics Symposium"}
@string{ectc = "Electronics Components and Technology Conference"}
@string{dmr = "IEEE Transactions on Device and Materials Reliability"}
@string{jep = "Journal of Electronic Packaging"}
@string{snsr = "IEEE Sensors Journal"}
@string{jap = "Journal of Applied Physics"}
@string{cambupress = "Cambridge University Press"}
@string{sispad = "International Conference on Simulation of Semiconductor Processes and Devices"}
@string{vtc = "IEEE Vehicular Technology Conference"}
@string{mnr= "Microelectronics Reliability"}
@string{nanotech = "IEEE Transactions on Nanotechnology"}
@string{apl = "Applied Physics Letters"}
@string{tmag = "IEEE Transactions on Magnetics"}
@string{apex = "Applied Physics Express"}
@string{trel = "IEEE Transactions on Reliability"}
@string{sse = "Solid-State Electronics"}
@string{jxcdc = "IEEE Journal on Exploratory Solid-State Computational Devices and Circuits"}
@string{cal = "IEEE Computer Architecture Letters"}
@string{spie = "SPIE Proceedings"}
@string{micro = "IEEE Micro"}
@string{vlsit = "Proceedings of the IEEE International Symposium on VLSI Technology"}
@string{asap = "Proceedings of the IEEE International Conference on Application-Specific Systems, Architectures and Processors"}
@string{hpdc = "Proceedings of the International Symposium on High-performance Parallel and Distributed Computing"}
@string{ics = "Proceedings of the 16th International Conference on Supercomputing"}
@string{ndp = "Workshop on Near-Data Processing in conjunction with the IEEE International Symposium on Microarchitecture"}
@string{microsymp = "IEEE International Symposium on Microarchitecture"}
@string{hbr = "Harvard Business Review"}
@string{icpp = "Proceedings of the International Conference on Parallel Processing"}, 
@string{icassp = "IEEE International Conference on Acoustics, Speech and Signal Processing"}
@string{tecs = "ACM Transactions on Embedded Computing Systems"}
@string{patmos = "Power and Timing Modeling, Optimization and Simulation (PATMOS)"}
@string{vlsisoc = "Proceedgins of the IFIP/IEEE International Conference on Very Large Scale Integration (VLSI-SoC)"}
@string{socc = "Proceedings of the IEEE International SOC Conference"}
@string{mse = "Proceedings of the IEEE International Conference on Microelectronic Systems Education"}
@string{glsvlsi = "Proceedings of the ACM Great Lakes Symposium on VLSI"},
@string{acmpd = "ACM International symposium on Physical Design"},
@string{iccv = "IEEE International Conference on Computer Vision"},
string{cad = "IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems"}
@string{comp = "IEEE Transactions on Computers"}
@string{cas = "IEEE Transactions on Circuits and Systems"}
@string{cas1 = "IEEE Transactions on Circuits and Systems I"}
@string{cas2 = "IEEE Transactions on Circuits and Systems II"}
@string{ibm = "IBM Journal of Research and Development"}
@string{ed = "IEEE Transactions on Electron Devices"}
@string{edl = "IEEE Electron Device Letters"}
@string{tvlsi = "IEEE Transactions on VLSI Systems"}
@string{cpmt = "IEEE Transactions on Components and Packaging Technologies"}
@string{tdmr = "IEEE Transactions on Devices and Materials Reliability"}
@string{solid = "IEEE Journal of Solid-State Circuits"}
@string{iccadold = "Proceedings of the IEEE International Conference on Computer-Aided Design"}
@string{iccad = "Proceedings of the IEEE/ACM International Conference on Computer-Aided Design"}
@string{dac = "Proceedings of the ACM/IEEE Design Automation Conference"}
@string{dacnew = "Proceedings of the ACM/EDAC/IEEE Design Automation Conference"}
@string{dacnewnew = "Proceedings of the ACM/ESDA/IEEE Design Automation Conference"}
@string{aspdac = "Proceedings of the Asia-South Pacific Design Automation Conference"}
@string{edac = "Proceedings of the European Design Automation Conference"}
@string{dateconf = "Proceedings of the Design, Automation \& Test in Europe"}
@string{iscas = "Proceedings of the IEEE International Symposium on Circuits and Systems"}
@string{itc = "Proceedings of the IEEE International Test Conference"}
@string{iccd = "Proceedings of the IEEE International Conference on Computer Design"}
@string{cicc = "Proceedings of the IEEE Custom Integrated Circuits Conference"}
@string{ieeepr = "Proceedings of the IEEE"}
@string{isscc = "Proceedings of the IEEE International Solid-State Circuits	Conference"}
@string{isqed = "Proceedings of the IEEE International Symposium on Quality Electronic Design"}
@string{edl = "IEEE Electron Device Letters"}
@string{ispd = "Proceedings of the International Symposium on Physical Design"}
@string{dnt = "IEEE Design \& Test"}
@string{islped = "Proceedings of the ACM International Symposium on Low Power Electronics and Design"}
@string{iedm = "IEEE International Electronic Devices Meeting"}
@string{irps = "Proceedings of the IEEE International Reliability Physics Symposium"}
@string{isca = "Proceedings of the ACM International Symposium on Computer Architecture"}
@string{todaes = "ACM Transactions on Design Automation of Electronic Systems"}
@string{ectc = "Electronics Components and Technology Conference"}
@string{dmr = "IEEE Transactions on Device and Materials Reliability"}
@string{jep = "Journal of Electronic Packaging"}
@string{snsr = "IEEE Sensors Journal"}
@string{jap = "Journal of Applied Physics"}
@string{cambupress = "Cambridge University Press"}
@string{ivtc = "Proceedings of the IEEE Vehicular Technology Conference"}
@string{icdm = "IEEE Circuits and Devices Magazine"}
@string{apl = "Applied Physics Letters"}
@string{icsspd= "International Conference on Simulation of Semiconductor Processes and Devices"}
@string{mr="Microelectronics Reliability"}
@string{me="Microelectronics Engineering"}
@string{mj="Microelectronics Journal"} % added by Vidya for asap7nm PDK
@string{pfaic="Proceedings of the International Symposium on the Physical and Failure Analysis of Integrated Circuits"}
@string{mse="IEEE International Conference on Microelectronic Systems  Education"}
@string{iitc="IEEE International Interconnect Technology Conference"}
@string{sispad="International Conference on Simulation of Semiconductor Processes and Devices"}
@string{jmr = "Journal of Materials Research"}
@string{chmt = "IEEE Transactions on Components Hybrids and Manufacturing Technology"}
@string{vlsisym = "IEEE Symposium on VLSI Technology"}
@string{ijeds="IEEE Journal of the Electron Devices Society"}
@string{iirw="Proceedings of the IEEE International Integrated Reliability Workshop"}
@string{iclr= "The International Conference on Learning Representations "}
@string{nips="Advances in Neural Information Processing Systems"}
@string{icicml = "Proceedings of the International Conference on International Conference on Machine Learning"}
@string{vlsidat = "Proceedings of the International Symposium on VLSI Design, Automation and Test"}
@string{fnt = "Foundations and Trends in Electronic Design Automation"}


@string{vlsisym = "IEEE Symp. VLSI Technol."}
@string{chmt = " IEEE Trans. Compon. Hybrids Manuf. Technol."} 
@string{dtc = " IEEE Des. Test Comput."} 
@string{cad = " IEEE T. Comput. Aid D."} 
@string{pami = "IEEE T. Pattern Anal. Mach. Intell."}
@string{tdmr = " IEEE T. Device Mater. Rel."} 
@string{jssc = " IEEE J. Solid-St. Circ."} 
@string{iccadold = " Proc. ICCAD"}  % IEEE IC CAD/ Proceedings of the IEEE International Conference on	Computer-Aided Design
@string{iccad = " Proc. ICCAD"} % ICCAD-IEEE ACM INT / Proceedings of the IEEE/ACM International Conference on Computer-Aided Design 
@string{dac = " Proc. DAC"} 
@string{dacnew = " Proc. DAC"} 
@string{dacnewnew = " Proc. DAC"} 
@string{aspdac = " Proc. ASP-DAC"} 
@string{dateconf = " Proc. DATE "}
@string{itc = " Proc. ITC"}
@string{cicc = " Proc. CICC"} 
@string{mr = " Microelectron. Reliab."} 
@string{me="Microelectron. Eng."}
@string{isqed = " Proc. ISQED"}  
@string{ispd = " Proc. ISPD"} 
@string{iedm = " Proc. IEDM"} 
@string{irps = "Proc. IRPS"}  
@string{jap = " J. Appl. Phys."} 
@string{vlsic = "Proc. VLSIC"}
@string{ddecs = "Proc. DDECS"}
@string{todaes = "ACM T. Des. Automat. El."}
@string{edl = "IEEE Electr. Device L."}
@string{tcad = "IEEE T. Comput. Aid. D."}
@string{tvlsi = "IEEE T. VLSI Syst"}
@string{tsemi = "IEEE T. Semiconduct. M."}
@string{cas2 = "IEEE T. Circuits-II"}
@string{cas1 = "IEEE T. CIRCUITS-I"}
@string{isca = "Proc. ISCA"}
@string{micro="Proc. MICRO"}
@string{iolts="Proc. IOLTS"}
@string{ibm = "IBM J. Res. Dev."}
@string{dnt = "IEEE Des. Test"}
@string{ed = "IEEE Trans. Electron Devices"}
@string{cal = "IEEE Comput. Archit. Lett."},
@string{ats = "Proc. ATS"}
@string{vts = "Proc. VTS"}
@string{rel = "IEEE T. Rel."}
@string{sigmetrics = "Proc. SIGMETRICS"},
@string{rams = "Proc. RAMS"}
@string{improc = "Proc. IEEE Int. Conf. Image Processing"}
@string{iccd = "Proc. ICCD"}
@string{dsn = "Proc. DSN"}
@string{sispad="Proc. SISPAD"}
@string{jmr = "J. Mater. Res."},
@string{iirw="Proc. IIRW"}, 
@string{iscas = "Proc. ISCAS"},
@string{iscas = "IEEE J. Electron Dev. Society"}
@string{ieeepr = "Proc. of the IEEE"}
@string{iclr = "Proc. ICLR"}
@string{icml = "Proc. ICML"}
@string{nips = "Proc. NeurIPS"}
@string{icicml = "Proc. ICICML"}
@string{vlsidat = "Proc. VLSI-DAT"}
@string{iciap = "Proc. Int. Conf. Image Analysis and Process."}
@string{eccv = "Proc. ECCV"}
@string{iccv = "Proc. ICCV"}
@string{cvpr = "Proc. CVPR"}
@string{fnt = "Found. Trends Electron. Des. Autom."}
@string{islped = "Proc. ISLPED"}


@INPROCEEDINGS{rl-sizer,
  author={Lu, Yi-Chen and Nath, Siddhartha and Khandelwal, Vishal and Lim, Sung Kyu},
  booktitle=dac, 
  title="{{RL-Sizer}: {VLSI} Gate Sizing for Timing Optimization using Deep Reinforcement Learning}", 
  year={2021},
  volume={},
  number={},
  pages={733-738},
  doi={10.1109/DAC18074.2021.9586138}}

@ARTICLE{chu1,
  author={Sharma, Ankur and Chinnery, David and Reimann, Tiago and Bhardwaj, Sarvesh and Chu, Chris},
  journal=cad, 
  title="{{Fast Lagrangian Relaxation-Based Multithreaded Gate Sizing Using Simple Timing Calibrations}}", 
  year={2020},
  volume={39},
  number={7},
  pages={1456-1469},
  doi={10.1109/TCAD.2019.2915324}}

@ARTICLE{chu2,
  author={C.-P. Chen and Chu, C.C.N. and Wong, D.F.},
  journal=cad, 
  title="{Fast and Exact Simultaneous Gate and Wire Sizing by Lagrangian Relaxation}", 
  year={1999},
  volume={18},
  number={7},
  pages={1014-1025},
  doi={10.1109/43.771182}}

@INPROCEEDINGS{chu3,  
author={Sharma, Ankur and Chinnery, David and Bhardwaj, Sarvesh and Chu, Chris},
booktitle=iccad,   
title="{{Fast Lagrangian Relaxation Based Gate Sizing using Multi-Threading}}",
year={2015},  
pages={426-433},  
doi={10.1109/ICCAD.2015.7372601}}


@incollection{pytorch,
title = "{{PyTorch:} An Imperative Style, High-Performance Deep Learning Library}",
author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and Desmaison, Alban and Kopf, Andreas and Yang, Edward and DeVito, Zachary and Raison, Martin and Tejani, Alykhan and Chilamkurthy, Sasank and Steiner, Benoit and Fang, Lu and Bai, Junjie and Chintala, Soumith},
booktitle = nips,
pages = {},
year = {2019},
}

@inproceedings{karypis20, 
title="{Deep Graph Library: A Graph-Centric, Highly-Performant Package for Graph Neural Networks}", 
author={Minjie Wang and Da Zheng and Zihao Ye and Quan Gan and Mufei Li and Xiang Song and Jinjing Zhou and Chao Ma and Lingfan Yu and Yu Gai and Tianjun Xiao and Tong He and George Karypis and Jinyang Li and Zheng Zhang},
booktitle="arXiv:1909.01315 [cs.ar]", 
year={2020},
volume={}, 
number={},
pages={}
}

@inproceedings{tilos,
  title={{TILOS: A Posynomial Programming Approach to Transistor Sizing}},
  author={J. P. Fishburn and A. E. Dunlop},
  booktitle=iccad,
  pages="326--328",
  year={1985}
}


@inproceedings{sensitivity-abk,
author = {Hu, J. and Kahng, A. B. and Kang, S. and Kim, M.-C. and Markov, I. L.},
title = "{Sensitivity-Guided Metaheuristics for Accurate Discrete Gate Sizing}",
year = {2012},
booktitle = iccad,
pages = "233--239",
numpages = {7},
location = {San Jose, California},
}

@inproceedings{10.1145/1077603.1077642,
author = {Chinnery, D. G. and Keutzer, K.},
title = {Linear Programming for Sizing, Vth and Vdd Assignment},
year = {2005},
booktitle = islped,
pages = {149–154}
}

@ARTICLE{convex,
  author={Kasamsetty, K. and Ketkar, M. and Sapatnekar, S.S.},
  journal=tcad, 
  title="{A New Class of Convex Functions for Delay Modeling and its Application to the Transistor Sizing Problem}", 
  year={2000},
  volume={19},
  number={7},
  pages={779-788},
  doi={10.1109/43.851993}}

@article{google-rl,
author = {Mirhoseini, Azalia and Goldie, Anna and Yazgan, Mustafa and Jiang, Joe and Songhori, Ebrahim and Shen, Wang and Lee, Young-Joon and Johnson, Eric and Pathak, Omkar and Nazi, Azade and Pak, Jiwoo and Tong, Andy and Srinivasa, Kavya and Hang, William and Tuncer, Emre and Le, Quoc and Laudon, James and Ho, Richard and Carpenter, Roger and Dean, Jeff},
year = {2021},
month = {06},
pages = {207-212},
title = "{A Graph Placement Methodology for Fast Chip Design}",
volume = {594},
journal = {Nature},
doi = {10.1038/s41586-021-03544-w}
}

@InProceedings{rgcn,
author="Schlichtkrull, Michael
and Kipf, Thomas N.
and Bloem, Peter
and van den Berg, Rianne
and Titov, Ivan
and Welling, Max",
title="{Modeling Relational Data with Graph Convolutional Networks}",
booktitle="The Semantic Web",
year="2018",
publisher="Springer",
pages="593--607",
isbn="978-3-319-93417-4"
}


@incollection{dqn,
  title = {{Playing Atari With Deep Reinforcement Learning}},
  author = {Volodymyr Mnih and Koray Kavukcuoglu and David Silver and Alex Graves and Ioannis Antonoglou and Daan Wierstra and Martin Riedmiller},
  booktitle = nips,
  year = {2013}
}

@misc{nangate45, 
title = {{NanGate 45nm FreePDK and Cell Library}},
year = 2022,
howpublished = {\url{https://si2.org/open-cell-library}}
}

@misc{orfs,
title = {{OpenROAD-flow-scripts}},
year = 2022,
howpublished = {\url{https://github.com/The-OpenROAD-Project/OpenROAD-flow-scripts}}
}


@misc{openroad,
title = {{OpenROAD}},
author = {},
year = 2022,
howpublished = {\url{https://github.com/The-OpenROAD-Project/OpenROAD}}
}


@misc{swig,
title = {{SWIG}},
author = {},
year = 2022,
howpublished = {\url{https://www.swig.org}}
}
`   
@misc{dc, 
title = {Synopsys {Design Compiler}},
year = 2022,
howpublished = {\url{"https://www.synopsys.com/implementation-and-signoff/rtl-synthesis-test.html"}}
}

@INPROCEEDINGS{survey-rl,
  author={Ren, Haoxing and Godil, Saad and Khailany, Brucek and Kirby, Robert and Liao, Haiguang and Nath, Siddhartha and Raiman, Jonathan and Roy, Rajarshi},
  booktitle=iccad, 
  title={{Optimizing VLSI Implementation with Reinforcement Learning}}, 
  year={2021}
  }

  @INPROCEEDINGS{lr-gnn-sizer,
  author={Zhou, Xinyi and Ye, Junjie and Pui, Chak-Wa and Shao, Kun and Zhang, Guangliang and Wang, Bin and Hao, Jianye and Chen, Guangyong and Heng, Phen Ann},
  booktitle=iccad, 
  title={{Heterogeneous Graph Neural Network-based Imitation Learning for Gate Sizing Acceleration}}, 
  year={2022}
  }



@InProceedings{mo-rl,
  title = 	 {{A Constrained Multi-Objective Reinforcement Learning Framework}},
  author =       {Huang, S. and others},
  booktitle = 	 {Proc. Conf. on Robot Learning},
  pages = 	 {883--893},
  year = 	 {2022}
}

@inproceedings{lp-sizer,
author = {Chinnery, D. G. and Keutzer, K.},
title = {{Linear Programming for Sizing, {Vth} and {Vdd} Assignment}},
year = {2005},
booktitle = islped,
pages = {149–154}
}

@inproceedings{fastplace,
author = {Viswanathan, Natarajan and Chu, Chris Chong-Nuen},
title = {{FastPlace: Efficient Analytical Placement Using Cell Shifting, Iterative Local Refinement and a Hybrid Net Model}},
year = {2004},
booktitle = ispd,
pages = {26–33},
numpages = {8},
}

@inproceedings{gcn-rl,
author = {Wang, Hanrui and Wang, Kuan and Yang, Jiacheng and Shen, Linxiao and Sun, Nan and Lee, Hae-Seung and Han, Song},
title = {{GCN-RL Circuit Designer: Transferable Transistor Sizing with Graph Neural Networks and Reinforcement Learning}},
year = {2020},
booktitle = dac,
numpages = {6},
}

@inproceedings{iscas85,
author = {Brglez, Franc and Fujiwara, Hideo},
year = {1985},
month = {06},
pages = {},
title = {{A Neutral Netlist of 10 Combinational Benchmark Circuits and a Targeted Translator in FORTRAN}}
}

@misc{rlblogpost,
    title={{Deep Reinforcement Learning Doesn't Work Yet}},
    author={Irpan, A.},
    howpublished={\url{https://www.alexirpan.com/2018/02/14/rl-hard.html}},
    year={2018}
}

@article{Chang13,
  author={Chang, H.-Y. and Jiang, I. H.-R. and Chang, Y.-W.},
  journal=tcad, 
  title={{ECO Optimization Using Metal-Configurable Gate-Array Spare Cells}}, 
  year={2013},
  volume={32},
  number={11},
  pages={1722-1733},
}

@article{Lee14,
author = {Lee, J. and Gupta, P.},
title = {{ECO Cost Measurement and Incremental Gate Sizing for Late Process Changes}},
year = {2013},
volume = {18},
number = {1},
journal = todaes,
month = {jan},
articleno = {16},
numpages = {11},
}

@INPROCEEDINGS{OpeNPDN,
    author={V. A. {Chhabria} and others},
    booktitle=aspdac, 
    title={Template-based {PDN} Synthesis in Floorplan and Placement Using   Classifier and {CNN} Techniques}, 
    year={2020},
    volume={},
    number={},
    pages={44--49},
}

@inproceeedings{Lin20,
author={Lin, H.-Y. and others},
  booktitle={Proc. ITC-Asia},
  title={Automatic IR-Drop ECO Using Machine Learning}, 
  year={2020},
  pages={7-12},
}

@book{BV09,
title = "Convex Optimization",
author = "S. Boyd and L. Vandenberghe",
publisher = "Cambridge University Press",
address = "Cambridge, UK",
year = 2009}

==> misc/customize.tex <==
\usepackage{float} 
\usepackage{tabularx}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{hhline}
\usepackage{silence}
\usepackage{graphicx}
\usepackage{multirow} 
\usepackage{graphicx}
\usepackage{multirow}
\usepackage[english]{babel}
\usepackage{booktabs}
\usepackage{array}
\usepackage{paralist}
\usepackage{threeparttable}
\usepackage{lipsum}
\usepackage{flushend}
\usepackage{cuted}
\usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage{algcompatible}
\usepackage{color}
\usepackage{psfrag}
\usepackage{epsfig}
\usepackage{multicol}
\usepackage{color}
\usepackage{fancybox}
\usepackage{subfigure}
\usepackage{cite}
\usepackage{theorem}
\usepackage{url}
\usepackage[table]{xcolor}
\usepackage{epstopdf}
\usepackage[normalem]{ulem}
\usepackage{siunitx}
\usepackage{rotating}

%\usepackage{biblatex} 
%\usepackage[backend=biber]{biblatex}
%\usepackage[style=apa,sortcites=true,sorting=nyt,backend=biber]{biblatex}
%\usepackage{subcaption}
\usepackage[justification=centering,font=small,labelfont=bf]{caption}
% \usepackage[font=small,labelfont=bf]{caption}
\usepackage{silence}
\WarningFilter{caption}{Unsupported document class}
\usepackage{enumitem}
%\usepackage{widetext}
%\usepackage{paralist}
%\usepackage[none]{hyphenat}
\definecolor{gray1}{gray}{0.90}
\definecolor{gray2}{gray}{0.98}
\definecolor{light-gray}{gray}{0.95}
\def\bibfont{\scriptsize}
%Adds extra padding to the table cells
\setlength\extrarowheight{2pt}

\newcommand{\ignore}[1]{}
\newcommand{\redHL}[1]{\textcolor{red}{#1}}
\newcommand{\blueHL}[1]{{\textcolor{blue}{#1}}}
\newcommand{\greenHL}[1]{\textcolor{green}{#1}}
\newcommand{\grayHL}[1]{\textcolor{gray}{#1}}
\newcommand{\blackHL}[1]{\textcolor{black}{#1}}
\newcommand{\redfn}[1]{\redHL{\footnote{\redHL{#1}}}
\newcommand{\Alter}[2]{\sout{#1}\redHL{#2}}
\newcommand{\txtoverline}[1]{$\overline{\mbox{{#1}}}$}
\newcommand{\TMR}{\mbox{TMR}}
\newcommand{\sTMR}{\scriptsize{\mbox{TMR}}}
%\newcommand{\Deff}{D_{\mbox{\tiny \em eff}}}
%\newcommand{\Deffn}{D_{\mbox{\tiny \em eff,n}}}
%\newcommand{\Deffg}{D_{\mbox{\tiny \em eff,g}}}
%\newcommand{\Zeff}{Z^\star_{\mbox{\tiny \em eff}}}
%\newcommand{\Javg}{J_{\mbox{\tiny \em avg}}}
%\newcommand{\Jeff}{J_{\mbox{\tiny \em eff}}}
%\newcommand{\Jrms}{J_{\mbox{\tiny \em rms}}}
%\newcommand{\Jflux}{J_{\mbox{\tiny \em flux}}}
%\newcommand{\vivekeq}[1]{\mbox{\tiny {\em #1}}}
%\newcommand{\Tlife}{T_{\mbox{\tiny \em life}}}
%\newcommand{\Ieff}{I_{\mbox{\tiny \em eff}}}
%\newcommand{\Irise}{I_{\mbox{\tiny \em rise}}}
%\newcommand{\Jpavg}{J_{\vivekeq{avg}}^+}
%\newcommand{\Jnavg}{J_{\vivekeq{avg}}^-}
%\newcommand{\Jbavg}{J_{\vivekeq{avg}}^{\vivekeq{blue}}}
%\newcommand{\Jgavg}{J_{\vivekeq{avg}}^{\vivekeq{green}}}
%\newcommand{\nuc}{t_{\mbox{\scriptsize \it nuc}}}
%\newcommand{\nucs}{t_{\mbox{\scriptsize \it nuc--SI}}}
%\newcommand{\nucf}{t_{\mbox{\scriptsize \it nuc--F}}}
%\newcommand{\tlife}{t_{\mbox{\scriptsize \it life}}}
%\newcommand{\Mx}{\mbox{M}_{\mbox{\scriptsize x}}}
%\newcommand{\Mxp}{\mbox{M}_{\mbox{\scriptsize x+1}}}
%\pagestyle{plain}
%\renewcommand{\bibfont}{\tiny}
\usepackage{tikz}
%\usetikzlibrary{tikzmark}
%\usetikzlibrary{shapes,arrows}
%\renewcommand{\baselinestretch}{0.93}
%\selectcolormodel{gray}


==> sec/algo_DQN.tex <==

\begin{algorithm}[!t]
\caption{RL-LR-Sizer DQN training}
\label{alg:training}
{\scriptsize
\begin{algorithmic}[1]
\State Initialize replay memory D to capacity N
\State Initialize action-value function $Q$ with random weights $W$
\State Initialize target action-value function $\hat{Q}$ with weights $\hat{W}$ = W
\For{episode = 1 : M}
    \State Reset $\mathrm{Env}$ and $s_t$ 
    \For{t = 1 : T}
        \If{ \textbf{With} Probability $\epsilon$}
            \State Select random valid action $a_t$
        \Else
            \State Select $a_t$ = $\mathrm{argmax}_a\;\phi(Q(s_t,a;W))$
%            \State Select $a_t$ = $\mathrm{argmax}_a\; (Q(s_t,a;W) \odot \mathrm{valid\_mask})$    
        \EndIf
        \State Execute action $a_t$ and update timing in $\mathrm{Env}$ 
        \State Calculate reward: \[R_t = L_{\lambda}(c^{t},slack^{t}) -L_{\lambda}(c^{t+1},slack^{t+1})\]
        \State Store transition($s_t,a_t,R_t,s_{t+1}$) in $D$
        \State Sample a random minibatch of  transition($s_j,a_j,R_j,s_{j+1}$) from $D$
        \State Set $y_j = 
        \begin{cases}
            R_j, & \text{if j is the last step}\\
            R_j + \gamma \max_{a'} \phi(\hat{Q}(s_{j+1},a';\hat{W})),              & \text{otherwise} \\
%            R_j + \gamma \max_{a'} (\hat{Q}(s_{j+1},a';\hat{W}) \odot \mathrm{action\_mask}),              & \text{Otherwise}
        \end{cases} $
        \State Gradient descent step on $(y_j - Q(s_j,a_j;W))^2$ with respect to $W$
        \If {$t$ mod $K == 0$}
         \For{$i \in \mathcal{I}$}
            \State $\lambda_i = \lambda_i\times (1-\frac{(slack_i)}{clock\,period})$ 
            \label{alg:lambda-update}
        \EndFor
        \EndIf
    \EndFor
    \If {$t$ mod $C == 0$}
        \State Reset $\hat{Q}=Q$
    \EndIf
    \State Decay $\epsilon$
\EndFor

\end{algorithmic}
}
\end{algorithm}



==> sec/old-2-background-LR.tex <==
\section{Problem formulation}
\label{sec:background-lr}

\noindent
The ECO problem is encountered late in the design cycle, after place-and-route and power grid design. 
% the physical design (PD) step is complete, i.. At this time, the netlist has been placed and routed and the power grid has been designed; however, due to limited interconnect resources, the supply grid is imperfect, i.e., its IR drop is higher than the allowable limit. As a result, 
Larger-than-expected IR drops result in increased gate delays, and the circuit fails timing. The ECO step resizes devices to bring the circuit back to timing specifications.  This involves both device upsizing (to improve drive strength) and downsizing (to reduce the load offered to the previous stage). In principle, upsizing/downsizing could change the current load and alter the voltage drop, but empirically, the change in current load is small, resulting in supply voltage changes (0.001\% of a 1.1V supply).

Formally, the objective of IR-aware ECO timing is to minimize the total power of the design while satisfying performance and electrical constraints after considering post-PD IR drop. 
% Timing constraints dictate that the circuit delay must be less than specified thresholds while the electrical constraints dictate that (i)~the effective capacitance load at the output pin  of a gate must be less than a specified limit, and (ii)~the slew at all input or output pins of a gate must be below a specification.\redfn{Should these constraints also be listed in the optimization problem below? Do we have LMs for these too?\blueHL{No we do not. This is an artifact of the old writeup where I first used DC to get an initial netlist which fixed slew and load violations then I sized cells using RL. I do not think we check these anymore.}} 
The constrained optimization problem is formulated as:
% \begin{align}
% % \begin{alignedat}{3}
%     \minimize \;&\; \textstyle \sum_{i\in\mathcal{I}} Area_{c_i} \;\; \label{eq:primal-problem} \\
%     \text{subject to}  \;&\; -\mathrm{slack}_i(V_{dd,i},GND_i) \le 0 \; \; \forall i \in \mathcal{I} \nonumber \\
%     % \;&\; \mathrm{load}_i \le \mathrm{max\_load}_{c_{i}} \;&\; \forall i \in \mathcal{I}\\
%     % \;&\; \mathrm{slew}_i \le \mathrm{max\_slew} \;&\; \forall i \in \mathcal{I}\\
%     \;&\; c_i \in \mathcal{C}_i \;\; \forall i \in \mathcal{I} \nonumber
% % \end{alignedat}
% \end{align}
\begin{align}
    \minimize \;&\; \textstyle \sum_{i\in\mathcal{I}} TotalPower_{c_i} \;\; \label{eq:primal-problem} \\
    \text{subject to}  \;&\; -\mathrm{slack}_i(V_{dd,i},GND_i) \le 0 \; \; \forall i \in \mathcal{I} \nonumber \\
    \;&\; c_i \in \mathcal{C}_i \;\; \forall i \in \mathcal{I} \nonumber
\end{align}
where $\mathcal{I}$ is a set of instances; $\mathcal{C}_i$ is the set of choices for instance $i$ in the library; $c_i \in \mathcal{C}_i$ is the library cell assigned to instance $i$; $\mathrm{TotalPower}_{c_i}$ is the total power consumption of instance $i$; and slack$_i$ is the slack at instance $i$ as a function of post-PD rail voltages, $V_{dd,i}$ and $GND_i$. The constraint on slack$_i$ uses ``$\le$'' form for nonnegative Lagrangian multipliers.

The primal problem~\eqref{eq:primal-problem}
% , when relaxed to a continuous problem, 
is translated~\cite{BV09} to an unconstrained problem using a nonnegative Lagrange multiplier (LM), $\lambda_i$, for each slack constraint, yielding the Lagrangian objective function:
% A modified version of the Lagrangian function, 
% $L_\lambda(c, \text{slack})$:
\begin{equation}
\boldsymbol{L_\lambda} (c,\mathrm{slack}): 
\textstyle
\sum_{i\in\mathcal{I}} TotalPower_{c_i} \\
+ \sum_{i\in\mathcal{I}} L_{slack,i}
%\lambda_i \times (- \mathrm{slack}_i)
\label{eq:objective}
\end{equation}
\begin{equation}
\mbox{where   }
L_{\text{slack},i} =
   \begin{cases} 
        \frac{\lambda_i (- \mathrm{slack}_i)}{\beta \times \mathrm{TNS} + \epsilon_0}   & \text{if $\mathrm{TNS} \leq \alpha\times\mathrm{clk}$ } \\ 
        \lambda_i (- \mathrm{slack}_i) & \text{otherwise} \\
    \end{cases}
\end{equation}
and $\boldsymbol{\lambda}$ is the vector of $\lambda_i$s.
Here, $\alpha$ and $\beta $ are tunable constants and $\beta < 0$, $\epsilon_0$ is a small value to prevent divide-by-zero; $\mathrm{clk}$ is the clock period; TNS is the sum of the negative slacks over all instances; and $c$ [$\mathrm{slack}$] is a set variable for $c_i$ [$\mathrm{slack}_i$]. We use $L_{\text{slack},i}$ to provide a higher importance to the slack component of the Langrangian as the slacks approach zero. This idea leads to the LR subproblem (LRS) formulation for gate sizing~\cite{chu1}, which, for a given $\boldsymbol{\lambda}$ is:
\begin{align}
\begin{alignedat}{3}
\mbox{\bf LRS:   }
  & \textstyle \minimize_{c,\mathrm{slack}} & L_\lambda(c,\mathrm{slack}) \\
  & \text{subject to} & c_i \in \mathcal{C}_i \;\; \forall i \in \mathcal{I}
\end{alignedat}
\label{eq:lr-subproblem}
\end{align}
LR solves the unconstrained problem~\eqref{eq:primal-problem}, iteratively updating the LMs $\boldsymbol{\lambda}$, and hence~\eqref{eq:lr-subproblem}, using a strategy described in Section~\ref{sec:rl-lr}.

We embed the above objective function into an RL framework as a reward and train an R-GCN agent to solve the LRS. \greyHL{Although we formulate the problem for power minimization, our approach can be applied to minimize area.} The LRS solver, which minimizes the weighted sum of slack and the total power (leakage + dynamic power) objective function.



\ignore{
\noindent
\redHL{\bf OLD VERSION BELOW THIS.}
\blueHL{The objective of IR-aware ECO timing is to minimize
the total area (or leakage power) of the
design while satisfying performance and electrical constraints after considering IR voltage drop. As the supply voltage decreases due to IR drop, the timing delays of logic gates increase. The excessive IR drop can lead to setup and hold time violation.}
% \redfn{Wenjing: you had listed ``setup and hold time violations'' earlier -- do you really see hold time violations due to larger IR drops? \blueHL{I just see setup violations. Let's not say hold violation here.} Increased IR drop $\Rightarrow$ increased delays, which can only hurt setup time constraints, not hold constraints.}
Timing constraints dictate that the circuit delay must be less than specified thresholds while the electrical constraints dictate that (i) the effective capacitance load at the output pin  of a gate must be less than a specified limit, and (ii) the slew at all input or output pins of a gate must not exceed a specified limit. The electrical constraints can easily be met with heuristic-based traversals of the netlist by inserting buffers and sizing logic gates locally.
% \redfn{Do we really insert buffers here? Or just size gates? \blueHL{Only gate sizing is involved in our experiment including preparing initial netlists by sizing-only model in DC and all flows.} And why do you say ``easily''? Isn't this the hard part that RL solves?\blueHL{I am also confused about the "easily" here which is in the old writeup and not changed. We may avoid say that.}}


\begin{equation}
\begin{alignedat}{3}
    \minimize_{c,\mathrm{slack}} \;&\; \sum_{i\in\mathcal{I}} Area_{c_i} \;&\; \\
    \text{subject to}  \;&\; -\mathrm{slack}_i \le 0 \;&\; \forall i \in \mathcal{I} \\
    % \;&\; \mathrm{load}_i \le \mathrm{max\_load}_{c_{i}} \;&\; \forall i \in \mathcal{I}\\
    % \;&\; \mathrm{slew}_i \le \mathrm{max\_slew} \;&\; \forall i \in \mathcal{I}\\
    \;&\; c_i \in \mathcal{C}_i \;&\; \forall i \in \mathcal{I}
    \label{eq:primal-problem}
\end{alignedat}
\end{equation}


\noindent
where $\mathcal{I}$ is  set of instances in the design, $\mathcal{C}_i$ is the set of choices for instance $i$ in the library, $c_i \in \mathcal{C}_i$ is the library cell assigned to instance $i$, and $\mathrm{Area}_{c_i}$ is the area of instance $i$.
% \redfn{Why the strange form (``$-$slack$_i \le 0$'') instead of the more normal ``slack$_i \ge 0$''?\blueHL{Vidya: any reason for this expression? In my memory, all constraints in an optimization problem are conventionally converted to use $\le$ or $=$, but I don't remember why. Vidya's comment: Constraint optimization problem forumated to minimize something with the Lagrangian multipliers. }} 

The primal problem~\eqref{eq:primal-problem}, when relaxed to a continuous problem, has nonconvex timing constraints. Therefore, we relax the problem by including those constraints into the objective function~\cite{chu1}. To penalize constraint violations, the slack constraint is associated  with a non-negative penalty coefficient.
The coefficient is called the Lagrange multiplier (LM)
and denoted by $\lambda_i$. Thus, we obtain a new objective function for a set of  $\boldsymbol{\lambda}$, called the Lagrangian function~\cite{chu1}. A modified version of the Lagrangian function, $L_\lambda(c, \text{slack})$ is shown below:

\begin{equation}
\boldsymbol{L_\lambda} (c,\mathrm{slack}): \sum_{i\in\mathcal{I}} Area_{c_i} \\
+ \sum_{i\in\mathcal{I}} L_{slack,i}
%\lambda_i \times (- \mathrm{slack}_i)
\end{equation}
\begin{equation}
\mbox{where   }
L_{\text{slack},i} =
   \begin{cases} 
        \frac{\lambda_i (- \mathrm{slack}_i)}{\beta \times \mathrm{TNS} + \epsilon_0}   & \text{if $\mathrm{TNS} \leq \alpha\times\mathrm{clk}$ } \\ 
        \lambda_i (- \mathrm{slack}_i) & \text{otherwise} \\
    \end{cases}
\end{equation}

\noindent
where $\alpha$ and $\beta $ are tunable constants and $\beta < 0$, $\epsilon_0$ is a small value to prevent a divide-by-zero condition, $\mathrm{clk}$ is the circuit clock period, and TNS is the sum of the negative slacks across all instances. We use $L_{\text{slack},i}$, as defined above, to provide a higher importance to the slack component of the Langrangian function as the slacks approach zero. Therefore, the LR subproblem for a given $\boldsymbol{\lambda}$ can be defined as:
\begin{equation}
\begin{alignedat}{3}
    \minimize_{c,\mathrm{slack}} \;&\; L_\lambda(c,\mathrm{slack}) \;&\; \\
    \text{subject to}  
    \;&\; c_i \in \mathcal{C}_i \;&\; \forall i \in \mathcal{I}
\end{alignedat}
\label{eq:lr-subproblem}
\end{equation}

\noindent
where $c$ and $\mathrm{slack}$ are the set variables for $c$ and $\mathrm{slack}$.

\blueHL{In our RL-LR ECO timing, we embed the above objective function into an RL framework as a reward and train an GCN agent to solve the LR subproblem.}
Although in this paper we formulate the problem for area minimization, our approach can be applied to minimize
leakage or dynamic power. The LRS solver, which minimizes the
weighted sum of slack and the leakage power, can be modified
to have leakage power or dynamic power as the objective.

%\redfn{Technically, I understand that LMs come from KKT, which applies to continuous optimization problems. Here, you have a discrete optimization problem, so at some point I assume there must be a relaxation of the problem to a continuous problem? Or am I missing something?~\blueHL{Yes I basically mention it in the paragraph above. Do I need to go into more details about KKT optimality conditions derivations?} {\em This isn't so much about KKT as about continuous vs. discrete (e.g., over a discrete space, there is no concept of a derivative, and therefore no KKT). As far as I can see, you talk about nonconvex timing constraints, but I don't see anything about how the discrete problem maps to this.}~\blueHL{Understood. Have not talked about how we went from discrete gate sizing problem to this formulation. This is based on our earlier email thread as well. The Chris Chu paper(s) does not explain this either. Perhaps we add a line saying we relax it to continuous?} Looks OK. Re Chris Chu -- he was solving the old problem where gate sizes were not necessarily discrete (or were rounded up somehow), which is why he could justify convexity (based on a posynomial formulation). So he did not have this problem.} 
}





==> sec/tbl-across-start-points-power-overhead-percentage.tex <==
\begin{table}
\centering
\caption{Results of multiple clock constraints for wb\_conmax}
\vspace{-4mm}
\label{tbl:across-points}
\resizebox{0.96\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c} 
\cline{1-6}
\multirow{3}{*}{Designs}     & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Target Delay\\(ns)\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Initial Delay\\(ns)\end{tabular}} & \multicolumn{3}{c|}{\% Power Overhead Savings}                                                                                                                                                                                                   &   \\ 
\cline{4-6}
                             &                                                                             &                                                                              & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}LR\\Baseline\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Inference across\\Timing Constraints\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}RL-LR ECO\\Training\end{tabular}} &   \\
                             &                                                                             &                                                                              &                                                                       &                                                                                               &                                                                          &   \\ 
\cline{1-6}
\multirow{5}{*}{wb\_conmax}  & 0.77                                                                        & 0.8337                                                                       & 11.76\%                                                               & 39.53\%                                                                                       & 45.27\%                                                                  &   \\ 
\cline{2-6}
                             & 0.79                                                                        & 0.8581                                                                       & 8.04\%                                                                & 10.28\%                                                                                       & 12.81\%                                                                  &   \\ 
\cline{2-6}
                             & 0.84                                                                        & 0.8855                                                                       & 71.73\%                                                               & 94.27\%                                                                                       & 88.81\%                                                                  &   \\ 
\cline{2-6}
                             & 0.86                                                                        & 0.9173                                                                       & 40.33\%                                                               & 60.53\%                                                                                       & 50.16\%                                                                  &   \\ 
\cline{2-6}
                             & 0.96                                                                        & 1.0002                                                                       & 71.45\%                                                               & 95.18\%                                                                                       & 90.09\%                                                                  &   \\ 
\cline{1-6}
\multicolumn{1}{|c}{Average} & \multicolumn{1}{c}{}                                                        & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{40.66\%}                                           & \multicolumn{1}{c}{59.96\%}                                                                   & 57.45\%                                                                  &   \\ 
\cline{1-6}
\multicolumn{1}{|c}{Maximum} & \multicolumn{1}{c}{}                                                        & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{71.73\%}                                           & \multicolumn{1}{c}{95.18\%}                                                                   & 90.09\%                                                                  &   \\
\cline{1-6}
\end{tabular}
}
\vspace{-2mm}
\end{table}

==> sec/tbl-across-start-points-power.tex <==
\begin{table}
\centering
\caption{Results of multiple start points for wb\_conmax}
\vspace{-4mm}
\label{tbl:across-points}
\resizebox{0.96\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c} 
\cline{1-6}
\multirow{3}{*}{Designs}     & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Target Delay\\(ns)\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Initial Delay\\(ns)\end{tabular}} & \multicolumn{3}{c|}{Power (mW)}                                                                                                                        &   \\ 
\cline{4-6}
                             &                                                                             &                                                                              & \multirow{2}{*}{LR}  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Inference across\\Timing Constraints\end{tabular}} & \multirow{2}{*}{RL-LR~Training} &   \\
                             &                                                                             &                                                                              &                      &                                                                                               &                                 &   \\ 
\cline{1-6}
\multirow{5}{*}{wb\_conmax}  & 0.77                                                                        & 0.8337                                                                       & 21.601               & 21.553 (-0.22\%)                                                                              & 21.454 (-0.68\%)                &   \\ 
\cline{2-6}
                             & 0.79                                                                        & 0.8581                                                                       & 20.818               & 20.714 (-0.50\%)                                                                              & 20.730 (-0.42\%)                &   \\ 
\cline{2-6}
                             & 0.84                                                                        & 0.8855                                                                       & 19.280               & 19.226 (-0.28\%)                                                                              & 19.239 (-0.21\%)                &   \\ 
\cline{2-6}
                             & 0.86                                                                        & 0.9173                                                                       & 19.084               & 19.008 (-0.40\%)                                                                              & 19.018 (-0.35\%)                &   \\ 
\cline{2-6}
                             & 0.96                                                                        & 1.0002                                                                       & 16.715               & 16.712 (-0.02\%)                                                                              & 16.715 (-0.00\%)                &   \\ 
\cline{1-6}
\multicolumn{1}{|c}{Average} & \multicolumn{1}{c}{}                                                        & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-0.28\%}                                                                   & -0.33\%                         &   \\ 
\cline{1-6}
\multicolumn{1}{|c}{Maximum} & \multicolumn{1}{c}{}                                                        & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-0.50\%}                                                                   & -0.68\%                         &   \\
\cline{1-6}
\end{tabular}
}
\vspace{-2mm}
\end{table}

==> sec/tbl-across-start-points.tex <==
\begin{table}
\centering
\caption{Results of mutiple start points for wb\_conmax design}
\vspace{-4mm}
\label{tbl:across-points}
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c} 
\cline{1-8}
\multirow{3}{*}{Designs}     & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Target Delay\\(ns)\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Initial Delay\\(ns)\end{tabular}} & \multicolumn{5}{c|}{Area($\mu$m$^2$)}                                                                                                                                                                                                         &   \\ 
\cline{4-8}
                             &                                                                             &                                                                              & \multirow{2}{*}{LR}  & \multicolumn{2}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Inference across\\Timing Constraints\end{tabular}}} & \multicolumn{2}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}RL-LR ECO\\Training\end{tabular}}} &   \\
                             &                                                                             &                                                                              &                      & \multicolumn{2}{c|}{}                                                                                              & \multicolumn{2}{c|}{}                                                                             &   \\ 
\cline{1-8}
\multirow{5}{*}{wb\_conmax}  & 0.77                                                                        & 0.8337                                                                       & 22297                & 22249                & 0.22\%                                                                                      & 22235                & 0.28\%                                                                     &   \\ 
\cline{2-8}
                             & 0.81                                                                        & 0.8581                                                                       & 22195                & 22130                & 0.29\%                                                                                      & 22108                & 0.39\%                                                                     &   \\ 
\cline{2-8}
                             & 0.85                                                                        & 0.8855                                                                       & 22097                & 22076                & 0.10\%                                                                                      & 22067                & 0.14\%                                                                     &   \\ 
\cline{2-8}
                             & 0.86                                                                        & 0.9173                                                                       & 22132                & 22077                & 0.25\%                                                                                      & 22065                & 0.30\%                                                                     &   \\ 
\cline{2-8}
                             & 0.96                                                                        & 1.0002                                                                       & 22046                & 22066                & -0.09\%                                                                                     & 22037                & 0.04\%                                                                     &   \\ 
\cline{1-8}
\multicolumn{1}{|c}{Average} & \multicolumn{1}{c}{}                                                        & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.15\%}                                                                  & \multicolumn{1}{c}{} & 0.23\%                                                                     &   \\ 
\cline{1-8}
\multicolumn{1}{|c}{Maximum} & \multicolumn{1}{c}{}                                                        & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.29\%}                                                                  & \multicolumn{1}{c}{} & 0.39\%                                                                     &   \\
\cline{1-8}
\end{tabular}
}
\vspace{-5mm}
\end{table}

==> sec/tbl-benchmarks.tex <==
\begin{table}[t]
\centering
\caption{\blueHL{IR-induced Timing Failure}}
\vspace{-4mm}
\label{tbl:benchmarks}
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|} 
\hline
\textbf{Design}  & \textbf{Target Period (ns)} & \textbf{\#Gates} & \textbf{\#Insts on Failed Paths}  \\ 
\hline
des\_area        & 0.56                        & 2100            & 129                              \\ 
\hline
wb\_dma          & 0.47                        & 2662            & 226                              \\ 
\hline
pid\_controller  & 0.75                        & 3536            & 182                              \\ 
\hline
aes\_cipher\_top & 0.88                        & 12421           & 1482                             \\ 
\hline
des\_perf        & 0.59                        & 21749           & 2110                             \\ 
\hline
pci\_bridge32    & 0.76                        & 22139           & 1142                             \\ 
\hline
wb\_conmax       & 0.80                        & 26228           & 1530                             \\
\hline
\end{tabular}
}
\vspace{-1.5em}
\end{table}

==> sec/tbl-results.tex <==

\begin{table}[t]
\centering
\caption{Metrics for designs in a 45nm technology for a specific clock.}
\label{tbl:results}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c| %design
>{\centering\arraybackslash}m{0.10\linewidth}| %delay
>{\centering\arraybackslash}m{0.12\linewidth}| %area
>{\centering\arraybackslash}m{0.16\linewidth}| %oper. clk period
>{\centering\arraybackslash}m{0.12\linewidth}| %area comm. tool
c| % area LR
c| % area RL
>{\centering\arraybackslash}m{0.08\linewidth}| %runtime LR
>{\centering\arraybackslash}m{0.13\linewidth}| %runtime RL
}
\hline
\multirow{2}{*}{{\bf Design}} & \multicolumn{2}{c|}{{\bf Initial}}& {\bf Operating} & \multicolumn{3}{c|}{{\bf Area ($um^2$)}} & \multicolumn{2}{c|}{{\bf Runtime}} \\ \cline{2-3} \cline{5-9} 
      & {\bf Delay} ($ns$) & {\bf Area ($um^2$)} & {\bf clk period} ($ns$)& {\bf Comm. tool} & {\bf LR}   & {\bf RL-LR}   & {\bf LR} (min) & {\bf RL-LR} (min) \\ \hline
c432  & 0.908        & 350.59        & 0.750     & 370.73     & 375.04    & 359.89  & 6   & 54  \\ \hline
c499  & 0.789        & 603.82        & 0.762     & 605.41     & 607.83    & 610.43  & 7  & 60  \\ \hline
c880  & 0.784        & 730.49        & 0.680     & 765.56     & 766.66    & 737.53  & 11    & 150  \\ \hline
c1355 & 0.836        & 780.16        & 0.770     & 822.34     & 811.60    & 799.25  & 14   & 162  \\ \hline
c1908 & 1.025        & 996.44        & 0.900     & 1044.47    & 1058.57   & 1023.99 & 18   & 168  \\ \hline
c2670 & 1.251        & 2785.28       & 1.100     & 2808.81    & 2817.48  & 2789.33  & 20   & 186   \\ \hline
c3540 & 1.586        & 1786.23       & 1.420     & 1829.98    & 1831.42   & 1805.50 & 21   & 210  \\ \hline
c5315 & 1.346        & 3491.11       & 1.212     & 3524.19    & 3522.93   & 3502.37 & 27   & 215  \\ \hline
c6288 & 3.750        & 2276.96       & 3.400     & 2353.39    & 2436.28   & 2304.54 & 33  & 262  \\ \hline
% gcd   & 0.556        &  503.23       & 0.515     & 511.28     & 508.84    & 505.52  & 4   & 50  \\ \hline
% {\bf Avg.}   & --       &  --       & --        & 1463.61    & 1473.67   & 1443.84  & 16  & 152 \\ \hline
\end{tabular}%
}
\vspace{-1.5em}
\end{table}


==> sec/tbl-transferbility-power-overhead.tex <==
\begin{table}
\centering
\caption{RL transferability across designs \blueHL{Power overhead savings}}
%\vspace{-4mm}
\label{tbl:across-designs}
\hspace*{-2mm}
\resizebox{1.1\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{IR Drop}                                                       & \multirow{2}{*}{Designs}           & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Target\\Delay\\(ns)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Initial\\Delay\\(ns)\end{tabular}} & \multicolumn{3}{c|}{Power Overhead Savings (mW)}                                                                                                       & \multicolumn{2}{c|}{Runtime(s)}                                                                                      \\ 
\cline{5-9}
                                                                               &                                    &                                                                              &                                                                               & LR                          & \begin{tabular}[c]{@{}c@{}}Inference across\\Designs\end{tabular} & \begin{tabular}[c]{@{}c@{}}Fine\\Tuning\end{tabular} & LR                   & \begin{tabular}[c]{@{}c@{}}Inference across Designs\\Or Fine Tuning (if needed)\end{tabular}  \\ 
\hline
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Low\\($\le$5mV)\end{tabular}}       & \textcolor{blue}{des\_area}        & 0.56                                                                         & 0.5676                                                                        & 0.202 (76.40\%)             & 0.208~(78.71\%)                                                   & NA                                                   & 55                   & 24 (-56.50\%)                                                                                 \\ 
\cline{2-9}
                                                                               & wb\_dma                            & 0.47                                                                         & 0.4859                                                                        & 0.060~(20.55\%)             & 0.061~(20.97\%)                                                   & NA                                                   & 39                   & 12 (-69.49\%)                                                                                 \\ 
\cline{2-9}
                                                                               & \textcolor{blue}{pid\_controller}  & 0.75                                                                         & 0.7641                                                                        & 0.139~(51.59\%)             & 0.140~(51.70\%)                                                   & NA                                                   & 54                   & 20 (-63.08\%)                                                                                 \\ 
\cline{2-9}
                                                                               & \textcolor{blue}{aes\_cipher\_top} & 0.89                                                                         & 0.9083                                                                        & 0.022~(4.26\%)              & 0.086~(16.67\%)                                                   & NA                                                   & 213                  & 121 (-43.09\%)                                                                                \\ 
\cline{2-9}
                                                                               & des\_perf                          & 0.59                                                                         & 0.6087                                                                        & 0.147~(14.27\%)             & 0.189~(18.35\%)                                                   & NA                                                   & 514                  & 142 (-72.37\%)                                                                                \\ 
\cline{2-9}
                                                                               & \textcolor{blue}{pci\_bridge32}    & 0.75                                                                         & 0.7718                                                                        & 0.087~(24.23\%)             & 0.088~(24.51\%)                                                   & NA                                                   & 185                  & 108 (-41.66\%)                                                                                \\ 
\cline{2-9}
                                                                               & wb\_conmax                         & 0.81                                                                         & 0.8286                                                                        & 0.229~(21.56\%)             & 0.253~(23.82\%)                                                   & NA                                                   & 274                  & 120 (-56.12\%)                                                                                \\ 
\hline
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Moderate\\($\le$10mV)\end{tabular}} & \textcolor{blue}{des\_area}        & 0.56                                                                         & 0.5896                                                                        & 0.134~(35.18\%)             & 0.174~(45.68\%)                                                   & NA                                                   & 82                   & 36 (-56.10\%)                                                                                 \\ 
\cline{2-9}
                                                                               & wb\_dma                            & 0.47                                                                         & 0.4859                                                                        & 0.048~(16.66\%)             & 0.055~(19.07\%)                                                   & NA                                                   & 47                   & 33 (-29.79\%)                                                                                 \\ 
\cline{2-9}
                                                                               & \textcolor{blue}{pid\_controller}  & 0.75                                                                         & 0.7814                                                                        & 0.134~(32.57\%)             & 0.139~(33.67\%)                                                   & NA                                                   & 58                   & 19 (-66.67\%)                                                                                 \\ 
\cline{2-9}
                                                                               & \textcolor{blue}{aes\_cipher\_top} & 0.89                                                                         & 0.9412                                                                        & 0.104~(8.60\%)              & 0.360~(29.78\%)                                                   & NA                                                   & 654                  & 94 (-85.63\%)                                                                                 \\ 
\cline{2-9}
                                                                               & des\_perf                          & 0.60                                                                         & 0.6318                                                                        & 0.197~(8.30\%)              & 0.269~(11.34\%)                                                   & NA                                                   & 576                  & 175 (-69.71\%)                                                                                \\ 
\cline{2-9}
                                                                               & \textcolor{blue}{pci\_bridge32}    & 0.75                                                                         & 0.7805                                                                        & 0.087~(15.96\%)             & 0.088~(16.15\%)                                                   & NA                                                   & 92                   & 15 (-83.88\%)                                                                                 \\ 
\cline{2-9}
                                                                               & wb\_conmax                         & 0.81                                                                         & 0.8581                                                                        & 0.149~(8.16\%)              & -                                                                 & 0.167 (9.14\%)                                       & 290                  & 331 (+13.97\%)                                                                                \\ 
\hline
\multicolumn{2}{|c}{Average}                                                                                        & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                                          & \multicolumn{1}{c}{24.17\%} & \multicolumn{1}{c}{30.03\%}                                       & \multicolumn{1}{c}{}                                 & \multicolumn{1}{c}{} &                                                                                               \\ 
\hline
\multicolumn{2}{|c}{Maximum}                                                                                        & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                                          & \multicolumn{1}{c}{76.40\%} & \multicolumn{1}{c}{78.71\%}                                       & \multicolumn{1}{c}{}                                 & \multicolumn{1}{c}{} &                                                                                               \\
\hline
\end{tabular}
}
%\vspace{-4mm}
\end{table}

==> sec/tbl-transferbility-power.tex <==
\begin{table}
\centering
\caption{RL transferability across designs}
\vspace{-4mm}
\label{tbl:across-designs}
\hspace*{-2mm}
\resizebox{1.1\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{IR Drop}                                                       & \multirow{2}{*}{Designs}           & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Target\\Delay\\(ns)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Initial\\Delay\\(ns)\end{tabular}} & \multicolumn{3}{c|}{Total Power (mW)}                                                                                                            & \multicolumn{2}{c|}{Runtime(s)}                                                                                      \\ 
\cline{5-9}
                                                                               &                                    &                                                                              &                                                                               & LR                   & \begin{tabular}[c]{@{}c@{}}Inference across\\Designs\end{tabular} & \begin{tabular}[c]{@{}c@{}}Fine\\Tuning\end{tabular} & LR                   & \begin{tabular}[c]{@{}c@{}}Inference across Designs\\Or Fine Tuning (if needed)\end{tabular}  \\ 
\hline
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Low\\($\le$5mV)\end{tabular}}       & \textcolor{blue}{des\_area}        & 0.56                                                                         & 0.5676                                                                        & 3.237                & 3.231 (-0.19\%)                                                   & NA                                                   & 55                   & 24 (-56.50\%)                                                                                 \\ 
\cline{2-9}
                                                                               & wb\_dma                            & 0.47                                                                         & 0.4859                                                                        & 8.030                & 8.029 (-0.01\%)                                                   & NA                                                   & 39                   & 12 (-69.49\%)                                                                                 \\ 
\cline{2-9}
                                                                               & \textcolor{blue}{pid\_controller}  & 0.75                                                                         & 0.7641                                                                        & 6.639                & 6.638 (-0.00\%)                                                   & NA                                                   & 54                   & 20 (-63.08\%)                                                                                 \\ 
\cline{2-9}
                                                                               & \textcolor{blue}{aes\_cipher\_top} & 0.89                                                                         & 0.9083                                                                        & 12.042               & 11.978 (-0.53\%)                                                  & NA                                                   & 213                  & 121 (-43.09\%)                                                                                \\ 
\cline{2-9}
                                                                               & des\_perf                          & 0.59                                                                         & 0.6087                                                                        & 30.001               & 29.959 (-0.14\%)                                                  & NA                                                   & 514                  & 142 (-72.37\%)                                                                                \\ 
\cline{2-9}
                                                                               & \textcolor{blue}{pci\_bridge32}    & 0.75                                                                         & 0.7718                                                                        & 17.458               & 17.457 (-0.01\%)                                                  & NA                                                   & 185                  & 108 (-41.66\%)                                                                                \\ 
\cline{2-9}
                                                                               & wb\_conmax                         & 0.81                                                                         & 0.8286                                                                        & 20.638               & 20.614 (-0.12\%)                                                  & NA                                                   & 274                  & 120 (-56.12\%)                                                                                \\ 
\hline
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Moderate\\($\le$10mV)\end{tabular}} & \textcolor{blue}{des\_area}        & 0.56                                                                         & 0.5896                                                                        & 3.305                & 3.265 (-1.21\%)                                                   & NA                                                   & 82                   & 36 (-56.10\%)                                                                                 \\ 
\cline{2-9}
                                                                               & wb\_dma                            & 0.47                                                                         & 0.4859                                                                        & 8.042                & 8.035 (-0.09\%)                                                   & NA                                                   & 47                   & 33 (-29.79\%)                                                                                 \\ 
\cline{2-9}
                                                                               & \textcolor{blue}{pid\_controller}  & 0.75                                                                         & 0.7814                                                                        & 6.644                & 6.639 (-0.07\%)                                                   & NA                                                   & 58                   & 19 (-66.67\%)                                                                                 \\ 
\cline{2-9}
                                                                               & \textcolor{blue}{aes\_cipher\_top} & 0.89                                                                         & 0.9412                                                                        & 12.260               & 12.004 (-2.09\%)                                                  & NA                                                   & 654                  & 94 (-85.63\%)                                                                                 \\ 
\cline{2-9}
                                                                               & des\_perf                          & 0.60                                                                         & 0.6318                                                                        & 30.251               & 30.179 (-0.24\%)                                                  & NA                                                   & 576                  & 175 (-69.71\%)                                                                                \\ 
\cline{2-9}
                                                                               & \textcolor{blue}{pci\_bridge32}    & 0.75                                                                         & 0.7805                                                                        & 17.458               & 17.457 (-0.01\%)                                                  & NA                                                   & 92                   & 15 (-83.88\%)                                                                                 \\ 
\cline{2-9}
                                                                               & wb\_conmax                         & 0.81                                                                         & 0.8581                                                                        & 20.818               & -                                                                 & 2.080E-02 (-0.09\%)                                  & 290                  & 331 (+13.97\%)                                                                                \\ 
\hline
\multicolumn{2}{|c}{Average}                                                                                        & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                                          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-0.36\%}                                       & \multicolumn{1}{c}{}                                 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}                                                                          \\ 
\hline
\multicolumn{2}{|c}{Maximum}                                                                                        & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                                          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-2.09\%}                                       & \multicolumn{1}{c}{}                                 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}                                                                          \\
\hline
\end{tabular}
}
\vspace{-4mm}
\end{table}

==> sec/tbl-transferbility.tex <==
\begin{table}
\centering
\caption{RL transferability across designs}
\vspace{-4mm}
\label{tbl:across-designs}
\hspace*{-2mm}
\resizebox{1.1\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{IR Drop}                                                       & \multirow{2}{*}{Designs}           & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Target\\Delay\\(ns)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Initial\\Delay\\(ns)\end{tabular}} & \multicolumn{5}{c|}{Area($\mu$m$^2$)}                                                                                                                                                     & \multicolumn{3}{c|}{Runtime(s)}                                                                                                           \\ 
\cline{5-12}
                                                                               &                                    &                                                                              &                                                                               & LR                   & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Inference across\\Designs\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Fine\\Tuning\end{tabular}} & LR                   & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Inference across Designs\\Or Fine Tuning (if needed)\end{tabular}}  \\ 
\hline
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Low\\($\le$5mV)\end{tabular}}       & \textcolor{blue}{des\_area}        & 0.56                                                                         & 0.5676                                                                        & 2411.6               & 2409.2               & 0.14\%                                                          & NA                   & NA                                                 & 57                   & 14                   & 75.40\%                                                                                     \\ 
\cline{2-12}
                                                                               & wb\_dma                            & 0.47                                                                         & 0.4859                                                                        & 4742.2               & 4741.2               & 0.02\%                                                          & NA                   & NA                                                 & 10                   & 13                   & -26.80\%                                                                                    \\ 
\cline{2-12}
                                                                               & \textcolor{blue}{pid\_controller}  & 0.75                                                                         & 0.7641                                                                        & 5508.9               & 5498.5               & 0.19\%                                                          & NA                   & NA                                                 & 112                  & 15                   & 86.29\%                                                                                     \\ 
\cline{2-12}
                                                                               & \textcolor{blue}{aes\_cipher\_top} & 0.89                                                                         & 0.9083                                                                        & 14502.0              & 14428.0              & 0.57\%                                                          & NA                   & NA                                                 & 79                   & 50                   & 36.46\%                                                                                     \\ 
\cline{2-12}
                                                                               & des\_perf                          & 0.59                                                                         & 0.6087                                                                        & 27125.0              & 27039.0              & 0.32\%                                                          & NA                   & NA                                                 & 319                  & 144                  & 54.86\%                                                                                     \\ 
\cline{2-12}
                                                                               & \textcolor{blue}{pci\_bridge32}    & 0.75                                                                         & 0.7718                                                                        & 25827.0              & 25826.0              & 0.00\%                                                          & NA                   & NA                                                 & 78                   & 11                   & 85.46\%                                                                                     \\ 
\cline{2-12}
                                                                               & wb\_conmax                         & 0.81                                                                         & 0.8286                                                                        & 22107.0              & 22074.0              & 0.15\%                                                          & NA                   & NA                                                 & 239                  & 13                   & 94.69\%                                                                                     \\ 
\hline
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Moderate\\($\le$10mV)\end{tabular}} & \textcolor{blue}{des\_area}        & 0.56                                                                         & 0.5896                                                                        & 2436.3               & 2426.5               & 0.40\%                                                          & NA                   & NA                                                 & 113                  & 37                   & 67.43\%                                                                                     \\ 
\cline{2-12}
                                                                               & wb\_dma                            & 0.47                                                                         & 0.4859                                                                        & 4748.1               & 4759.8               & -0.25\%                                                         & NA                   & NA                                                 & 29                   & 23                   & 19.31\%                                                                                     \\ 
\cline{2-12}
                                                                               & \textcolor{blue}{pid\_controller}  & 0.75                                                                         & 0.7814                                                                        & 5520.3               & 5500.3               & 0.36\%                                                          & NA                   & NA                                                 & 107                  & 19                   & 81.93\%                                                                                     \\ 
\cline{2-12}
                                                                               & \textcolor{blue}{aes\_cipher\_top} & 0.89                                                                         & 0.9412                                                                        & 14799.0              & 14479.0              & 2.16\%                                                          & NA                   & NA                                                 & 255                  & 129                  & 49.21\%                                                                                     \\ 
\cline{2-12}
                                                                               & des\_perf                          & 0.60                                                                         & 0.6318                                                                        & 27454.0              & --                   & --                                                              & 27174.0              & 1.02\%                                             & 354                  & 458                  & -29.38\%                                                                                    \\ 
\cline{2-12}
                                                                               & \textcolor{blue}{pci\_bridge32}    & 0.75                                                                         & 0.7805                                                                        & 25828.0              & 25827.0              & 0.00\%                                                          & NA                   & NA                                                 & 78                   & 13                   & 83.64\%                                                                                     \\ 
\cline{2-12}
                                                                               & wb\_conmax                         & 0.81                                                                         & 0.8581                                                                        & 22195.0              & --                   & --                                                              & 22145.0              & 0.23\%                                             & 241                  & 493                  & -104.56\%                                                                                   \\ 
\hline
\multicolumn{2}{|c}{Average}                                                                                        & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                                          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.34\%}                                      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.37\%}                         & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &                                                                                             \\ 
\hline
\multicolumn{2}{|c}{Maximum}                                                                                        & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                                          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{2.16\%}                                      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{1.02\%}                         & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &                                                                                             \\
\hline
\end{tabular}
}
\vspace{-4mm}
\end{table}

==> sec/tbl-within-design-area-to-power.tex <==
\begin{table*}[t]
\centering
% \vspace{-6mm}
\caption{ECO timing result comparison for three different flows in \blueHL{power}, runtime, cell change metrics}
\vspace{-4mm}
\label{tbl:within-design-10mV-power}
\hspace*{-2mm}
%\resizebox{1.05\linewidth}{!}{
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{Designs}     & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Target\\Delay\\(ns)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Initial\\Delay\\(ns)\end{tabular}} & \multicolumn{5}{c|}{Dynamic/Leakage Power(W)}                                                                                                                                                              & \multicolumn{4}{c|}{Runtime(s)}                                                                                                                                                     & \multicolumn{3}{c|}{\# of Upsize/Downsize}                                                                                                                     \\ 
\cline{4-15}
                             &                                                                              &                                                                               & LR                      & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Inference across\\Timing Constraints\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}RL-LR\\Training\end{tabular}} & LR                   & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Inference~across \\Timing Constraints\end{tabular}} & \begin{tabular}[c]{@{}c@{}}RL-LR\\Training\end{tabular} & LR                   & \begin{tabular}[c]{@{}c@{}}Inference~across\\Timing Constraints\end{tabular} & \begin{tabular}[c]{@{}c@{}}RL-LR\\Training\end{tabular}  \\ 
\hline
des\_area                    & 0.56                                                                         & 0.5896                                                                        & 1.4400E-03 /~5.6400E-05 & 1.4900E-03 /~~5.7300E-05 & -3.47\% /~-1.60\%                                                      & 1.4300E-03 /~5.6000E-05 & 0.69\% / 0.71\%~                                   & 113                  & 33                   & 70.80\%                                                                     & 2251                                                    & 48/1                 & 74/2                                                                         & 26/4                                                     \\ 
\hline
wb\_dma                      & 0.47                                                                         & 0.4859                                                                        & 1.3041E-03 /~9.2947E-05 & 1.3032E-03 /~9.2953E-05  & 0.07\% /~-0.01\%                                                       & 1.3054E-03 /~9.2947E-05 & -0.10\% /~0.00\%                                   & 29                   & 14                   & 51.72\%                                                                     & 2285                                                    & 12/0                 & 9/0                                                                          & 8/3                                                      \\ 
\hline
pid\_controller              & 0.75                                                                         & 0.7814                                                                        & 2.2245E-03 /~1.0308E-04 & 2.2206E-03 /~1.0264E-04  & 0.18\% /~0.43\%                                                        & 2.2284E-03 /~1.0281E-04 & -0.18\% /~0.26\%                                   & 107                  & 26                   & 75.76\%                                                                     & 2718                                                    & 29/2                 & 25/4                                                                         & 26/6                                                     \\ 
\hline
aes\_cipher\_top             & 0.89                                                                         & 0.9412                                                                        & 5.1093E-03 /~3.0890E-04 & 4.9730E-03 /~3.0139E-04  & 2.67\% / 2.43\%                                                        & 4.9731E-03 /~3.0044E-04 & 2.67\% / 2.74\%                                    & 127                  & 113                  & 55.52\%                                                                     & 3015                                                    & 386/3                & 99/0                                                                         & 103/1                                                    \\ 
\hline
des\_perf                    & 0.60                                                                         & 0.6318                                                                        & 8.3766E-03 /~5.9502E-04 & 8.2799E-03 /~5.8960E-04  & 1.15\%~/ 0.91\%                                                        & 8.2343E-03/~5.8687E-04  & 1.70\% / 1.37\%                                    & 354                  & 103                  & 70.79\%                                                                     & 3103                                                    & 347/1                & 230/0                                                                        & 185/1                                                    \\ 
\hline
pci\_bridge32                & 0.75                                                                         & 0.7805                                                                        & 2.8222E-03 /~4.5167E-04 & 2.8206E-03 /~4.5160E-04  & 0.04\% /~0.02\%                                                        & 2.8211E-03 /~4.5158E-04 & 0.06\% / 0.02\%                                    & 78                   & 51                   & 34.19\%                                                                     & 2794                                                    & 24/1                 & 21/1                                                                         & 24/3                                                     \\ 
\hline
wb\_conmax                   & 0.81                                                                         & 0.8581                                                                        & 7.5837E-03 /~4.6985E-04 & 7.4903E-03 /~4.6822E-04  & 1.23\% /~0.35\%                                                        & 7.4864E-03 /~4.6755E-04 & 1.28\% /~~0.49\%                                   & 241                  & 125                  & 48.13\%                                                                     & 3123                                                    & 81/0                 & 55/0                                                                         & 45/2                                                     \\ 
\hline
\multicolumn{1}{|c}{Average} & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                                          & \multicolumn{1}{c}{}    & \multicolumn{1}{c}{}     & \multicolumn{1}{c}{0.27\% /~0.36\%}                                    & \multicolumn{1}{c}{}    & \multicolumn{1}{c}{0.87\% /~0.80\%}                & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{58.13\%}                                                 & \multicolumn{1}{c}{}                                    & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}                                                         &                                                          \\ 
\hline
\multicolumn{1}{|c}{Maximum} & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                                          & \multicolumn{1}{c}{}    & \multicolumn{1}{c}{}     & \multicolumn{1}{c}{2.67\% /~2.43\%}                                    & \multicolumn{1}{c}{}    & \multicolumn{1}{c}{2.67\% / 2.74\%}                & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{75.76\%}                                                 & \multicolumn{1}{c}{}                                    & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}                                                         &                                                          \\
\hline
\end{tabular}
}
\vspace{-2mm}
\end{table*}

==> sec/tbl-within-design-power-minsize-baseline.tex <==
\begin{table*}[t]
\centering
% \vspace{-6mm}
\caption{ECO timing result comparison for three different flows in power, runtime, cell change metrics\blueHL{(minsize baseline)}}
\vspace{-4mm}
\label{tbl:within-design-10mV-power}
\hspace*{-2mm}
%\resizebox{1.05\linewidth}{!}{
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{Designs}     & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Target\\Delay\\(ns)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Initial\\Delay\\(ns)\end{tabular}} & \multicolumn{5}{c|}{Power Overhead (mW)}                                                                                                                                                                    & \multicolumn{4}{c|}{Runtime(s)}                                                                                                                                                     & \multicolumn{3}{c|}{\# of Upsize/Downsize}                                                                                                                     \\ 
\cline{4-15}
                             &                                                                              &                                                                               & LR                   & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Inference across\\Timing Constraints\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}RL-LR\\Training\end{tabular}} & LR                   & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Inference~across \\Timing Constraints\end{tabular}} & \begin{tabular}[c]{@{}c@{}}RL-LR\\Training\end{tabular} & LR                   & \begin{tabular}[c]{@{}c@{}}Inference~across\\Timing Constraints\end{tabular} & \begin{tabular}[c]{@{}c@{}}RL-LR\\Training\end{tabular}  \\ 
\hline
des\_area                    & 0.56                                                                         & 0.5896                                                                        & 0.605                & 0.599                & 1.12\%                                                                     & 0.553                & 8.57\%                                                & 82                   & 23                   & 71.95\%                                                                     & 2651                                                    & 29/0                 & 36/6                                                                         & 27/4                                                     \\ 
\hline
wb\_dma                      & 0.47                                                                         & 0.4859                                                                        & 2.142                & 2.135                & 0.30\%                                                                     & 2.133                & 0.41\%                                                & 47                   & 42                   & 10.64\%                                                                     & 2284                                                    & 12/0                 & 19/0                                                                         & 18/3                                                     \\ 
\hline
pid\_controller              & 0.75                                                                         & 0.7814                                                                        & 2.644                & 2.641                & 0.11\%                                                                     & 2.639                & 0.17\%                                                & 58                   & 21                   & 63.79\%                                                                     & 2881                                                    & 29/2                 & 29/2                                                                         & 20/9                                                     \\ 
\hline
aes\_cipher\_top             & 0.89                                                                         & 0.9412                                                                        & 0.460                & 0.397                & 13.70\%                                                                    & 0.235                & 48.91\%                                               & 654                  & 153                  & 76.61\%                                                                     & 2305                                                    & 386/3                & 301/3                                                                        & 291/1                                                    \\ 
\hline
des\_perf                    & 0.60                                                                         & 0.6318                                                                        & 1.221                & 1.047                & 14.25\%                                                                    & 1.114                & 8.76\%                                                & 576                  & 398                  & 30.94\%                                                                     & 2322                                                    & 491/1                & 393/1                                                                        & 380/5                                                    \\ 
\hline
pci\_bridge32                & 0.75                                                                         & 0.7805                                                                        & 4.958                & 4.958                & 0.00\%                                                                     & 4.957                & 0.02\%                                                & 92                   & 54                   & 41.30\%                                                                     & 2336                                                    & 24/1                 & 22/1                                                                         & 23/1                                                     \\ 
\hline
wb\_conmax                   & 0.79                                                                         & 0.8581                                                                        & 1.418                & 1.314                & 7.33\%                                                                     & 1.333                & 5.99\%                                                & 290                  & 242                  & 16.55\%                                                                     & 3193                                                    & 86/0                 & 78/0                                                                         & 73/0                                                     \\ 
\hline
\multicolumn{1}{|c}{Average} & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                                          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}                                                       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}                                  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{44.54\%}                                                 & \multicolumn{1}{c}{}                                    & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}                                                         &                                                          \\ 
\hline
\multicolumn{1}{|c}{Maximum} & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                                          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}                                                       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}                                  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{76.61\%}                                                 & \multicolumn{1}{c}{}                                    & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}                                                         &                                                          \\
\hline
\end{tabular}
}
\vspace{-2mm}
\end{table*}

==> sec/tbl-within-design-power-overhead-percentage.tex <==
\begin{table*}[t]
\centering
% \vspace{-6mm}
\caption{ECO timing result comparison for three different flows in power, runtime, cell change metrics}
\vspace{-4mm}
\label{tbl:within-design-10mV-power}
\hspace*{-2mm}
%\resizebox{1.05\linewidth}{!}{
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{Designs}     & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Target\\Delay\\(ns)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Initial\\Delay\\(ns)\end{tabular}} & \multicolumn{3}{c|}{\% Power Overhead Savings}                                                                                                                                                    & \multicolumn{3}{c|}{Runtime(s)}                                                                                                                                                                    & \multicolumn{3}{c|}{\# of Upsize/Downsize}                                                                                                                                                         \\ 
\cline{4-12}
                             &                                                                              &                                                                               & \begin{tabular}[c]{@{}c@{}}LR\\Baseline\end{tabular} & \begin{tabular}[c]{@{}c@{}}Inference across\\Timing Constraints\end{tabular} & \begin{tabular}[c]{@{}c@{}}RL-LR ECO\\Training\end{tabular} & \begin{tabular}[c]{@{}c@{}}LR\\Baseline\end{tabular} & \begin{tabular}[c]{@{}c@{}}Inference~across \\Timing Constraints\end{tabular} & \begin{tabular}[c]{@{}c@{}}RL-LR ECO\\Training\end{tabular} & \begin{tabular}[c]{@{}c@{}}LR\\Baseline\end{tabular} & \begin{tabular}[c]{@{}c@{}}Inference~across\\Timing Constraints\end{tabular} & \begin{tabular}[c]{@{}c@{}}RL-LR ECO\\Training\end{tabular}  \\ 
\hline
des\_area                    & 0.56                                                                         & 0.5896                                                                        & 35.18\%                                              & 36.97\%                                                                      & 48.84\%                                                     & 82                                                   & 23 (-71.95\%)                                                                 & 2651                                                        & 29/0                                                 & 36/6                                                                         & 27/4                                                         \\ 
\hline
wb\_dma                      & 0.47                                                                         & 0.4859                                                                        & 16.66\%                                              & 18.90\%                                                                      & 19.66\%                                                     & 47                                                   & 42 (-10.64\%)                                                                 & 2284                                                        & 12/0                                                 & 19/0                                                                         & 18/3                                                         \\ 
\hline
pid\_controller              & 0.75                                                                         & 0.7814                                                                        & 32.57\%                                              & 33.28\%                                                                      & 33.67\%                                                     & 58                                                   & 21~(-63.79\%)                                                                 & 2881                                                        & 29/2                                                 & 29/2                                                                         & 20/9                                                         \\ 
\hline
aes\_cipher\_top             & 0.89                                                                         & 0.9412                                                                        & 8.60\%                                               & 13.81\%                                                                      & 27.21\%                                                     & 654                                                  & 153~(-76.61\%)                                                                & 2305                                                        & 386/3                                                & 301/3                                                                        & 291/1                                                        \\ 
\hline
des\_perf                    & 0.60                                                                         & 0.6318                                                                        & 8.30\%                                               & 15.63\%                                                                      & 12.81\%                                                     & 576                                                  & 398~(-30.94\%)                                                                & 2322                                                        & 491/1                                                & 393/1                                                                        & 380/5                                                        \\ 
\hline
pci\_bridge32                & 0.75                                                                         & 0.7805                                                                        & 15.96\%                                              & 15.96\%                                                                      & 16.15\%                                                     & 92                                                   & 54~(-41.30\%)                                                                 & 2336                                                        & 24/1                                                 & 22/1                                                                         & 23/1                                                         \\ 
\hline
wb\_conmax                   & 0.77                                                                         & 0.8337                                                                        & 11.76\%                                              & 39.53\%                                                                      & 45.27\%                                                     & 290                                                  & 242~(-16.55\%)                                                                & 3193                                                        & 86/0                                                 & 78/0                                                                         & 73/0                                                         \\ 
\hline
\multicolumn{1}{|c}{Average} & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                                          & \multicolumn{1}{c}{18.43\%}                          & \multicolumn{1}{c}{24.87\%}                                                  & \multicolumn{1}{c}{29.09\%}                                 & \multicolumn{1}{c}{}                                 & \multicolumn{1}{c}{-44.54\%}                                                  & \multicolumn{1}{c}{}                                        & \multicolumn{1}{c}{}                                 & \multicolumn{1}{c}{+3.27\%}                                                  & -7.78\%                                                      \\ 
\hline
\multicolumn{1}{|c}{Maximum} & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                                          & \multicolumn{1}{c}{35.18\%}                          & \multicolumn{1}{c}{39.53\%}                                                  & \multicolumn{1}{c}{48.84\%}                                 & \multicolumn{1}{c}{}                                 & \multicolumn{1}{c}{-76.61\%}                                                  & \multicolumn{1}{c}{}                                        & \multicolumn{1}{c}{}                                 & \multicolumn{1}{c}{-22.02\%}                                                 & -31.03\%                                                     \\
\hline
\end{tabular}
}
\vspace{-2mm}
\end{table*}

==> sec/tbl-within-design-power-overhead.tex <==
\begin{table*}[t]
\centering
% \vspace{-6mm}
\caption{ECO timing result comparison for three different flows in power, runtime, cell change metrics\blueHL{(Power overhead savings)}}
\vspace{-4mm}
\label{tbl:within-design-10mV-power}
\hspace*{-2mm}
%\resizebox{1.05\linewidth}{!}{
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{Designs}     & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Target\\Delay\\(ns)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Initial\\Delay\\(ns)\end{tabular}} & \multicolumn{3}{c|}{Power Overhead Savings (mW)}                                                                                                               & \multicolumn{3}{c|}{Runtime(s)}                                                                                                                                & \multicolumn{3}{c|}{\# of Upsize/Downsize}                                                                                                                     \\ 
\cline{4-12}
                             &                                                                              &                                                                               & LR                   & \begin{tabular}[c]{@{}c@{}}Inference across\\Timing Constraints\end{tabular} & \begin{tabular}[c]{@{}c@{}}RL-LR\\Training\end{tabular} & LR                   & \begin{tabular}[c]{@{}c@{}}Inference~across \\Timing Constraints\end{tabular} & \begin{tabular}[c]{@{}c@{}}RL-LR\\Training\end{tabular} & LR                   & \begin{tabular}[c]{@{}c@{}}Inference~across\\Timing Constraints\end{tabular} & \begin{tabular}[c]{@{}c@{}}RL-LR\\Training\end{tabular}  \\ 
\hline
des\_area                    & 0.56                                                                         & 0.5896                                                                        & 0.134 (35.18\%)      & 0.141 (36.97\%)                                                              & 0.186 (48.84\%)                                         & 82                   & 23 (-71.95\%)                                                                 & 2651                                                    & 29/0                 & 36/6                                                                         & 27/4                                                     \\ 
\hline
wb\_dma                      & 0.47                                                                         & 0.4859                                                                        & 0.048 (16.66\%)      & 0.055 (18.90\%)                                                              & 0.057 (19.66\%)                                         & 47                   & 42 (-10.64\%)                                                                 & 2284                                                    & 12/0                 & 19/0                                                                         & 18/3                                                     \\ 
\hline
pid\_controller              & 0.75                                                                         & 0.7814                                                                        & 0.134 (32.57\%)      & 0.137 (33.28\%)                                                              & 0.139 (33.67\%)                                         & 58                   & 21~(-63.79\%)                                                                 & 2881                                                    & 29/2                 & 29/2                                                                         & 20/9                                                     \\ 
\hline
aes\_cipher\_top             & 0.89                                                                         & 0.9412                                                                        & 0.104 (8.60\%)       & 0.167 (13.81\%)                                                              & 0.329 (27.21\%)                                         & 654                  & 153~(-76.61\%)                                                                & 2305                                                    & 386/3                & 301/3                                                                        & 291/1                                                    \\ 
\hline
des\_perf                    & 0.60                                                                         & 0.6318                                                                        & 0.197 (8.30\%)       & 0.371 (15.63\%)                                                              & 0.304 (12.81\%)                                         & 576                  & 398~(-30.94\%)                                                                & 2322                                                    & 491/1                & 393/1                                                                        & 380/5                                                    \\ 
\hline
pci\_bridge32                & 0.75                                                                         & 0.7805                                                                        & 0.087 (15.96\%)      & 0.087 (15.96\%)                                                              & 0.088 (16.15\%)                                         & 92                   & 54~(-41.30\%)                                                                 & 2336                                                    & 24/1                 & 22/1                                                                         & 23/1                                                     \\ 
\hline
wb\_conmax                   & 0.81                                                                         & 0.8581                                                                        & 0.149 (8.16\%)       & 0.253 (13.85\%)                                                              & 0.234 (12.81\%)                                         & 290                  & 242~(-16.55\%)                                                                & 3193                                                    & 86/0                 & 78/0                                                                         & 73/0                                                     \\ 
\hline
\multicolumn{1}{|c}{Average} & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                                          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                    & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-44.54\%}                                                  & \multicolumn{1}{c}{}                                    & \multicolumn{1}{c}{} & \multicolumn{1}{c}{+3.27\%}                                                  & -7.78\%                                                  \\ 
\hline
\multicolumn{1}{|c}{Maximum} & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                                          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                    & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-76.61\%}                                                  & \multicolumn{1}{c}{}                                    & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-22.02\%}                                                 & -31.03\%                                                 \\
\hline
\end{tabular}
}
\vspace{-2mm}
\end{table*}

==> sec/tbl-within-design-power.tex <==
\begin{table*}[t]
\centering
% \vspace{-6mm}
\caption{ECO timing result comparison for three different flows in power, runtime, cell change metrics}
\vspace{-4mm}
\label{tbl:within-design-10mV-power-minsize-baseline}
\hspace*{-2mm}
%\resizebox{1.05\linewidth}{!}{
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{Designs}     & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Target\\Delay\\(ns)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Initial\\Delay\\(ns)\end{tabular}} & \multicolumn{3}{c|}{Total Power(mW)}                                                                                                                          & \multicolumn{3}{c|}{Runtime(s)}                                                                                                                                & \multicolumn{3}{c|}{\# Upsize/Downsize Operations}                                                                                                             \\ 
\cline{4-12}
                             &                                                                              &                                                                               & LR                   & \begin{tabular}[c]{@{}c@{}}Inference across\\Timing Constraints\end{tabular} & \begin{tabular}[c]{@{}c@{}}RL-LR\\Training\end{tabular} & LR                   & \begin{tabular}[c]{@{}c@{}}Inference~across \\Timing Constraints\end{tabular} & \begin{tabular}[c]{@{}c@{}}RL-LR\\Training\end{tabular} & LR                   & \begin{tabular}[c]{@{}c@{}}Inference~across\\Timing Constraints\end{tabular} & \begin{tabular}[c]{@{}c@{}}RL-LR\\Training\end{tabular}  \\ 
\hline
des\_area                    & 0.56                                                                         & 0.5896                                                                        & 3.305                & 3.299 (-0.21\%)                                                              & 3.253 (-1.57\%)                                         & 82                   & 23 (-71.95\%)                                                                 & 2651                                                    & 29/0                 & 36/6                                                                         & 27/4                                                     \\ 
\hline
wb\_dma                      & 0.47                                                                         & 0.4859                                                                        & 8.042                & 8.035 (-0.08\%)                                                              & 8.033 (-0.11\%)                                         & 47                   & 42 (-10.64\%)                                                                 & 2284                                                    & 12/0                 & 19/0                                                                         & 18/3                                                     \\ 
\hline
pid\_controller              & 0.75                                                                         & 0.7814                                                                        & 6.644                & 6.641 (-0.04\%)                                                              & 6.639 (-0.07\%)                                         & 58                   & 21 (-63.79\%)                                                                 & 2881                                                    & 29/2                 & 29/2                                                                         & 20/9                                                     \\ 
\hline
aes\_cipher\_top             & 0.89                                                                         & 0.9412                                                                        & 12.260               & 12.197 (-0.51\%)                                                             & 12.035 (-1.84\%)                                        & 654                  & 153 (-76.61\%)                                                                & 2305                                                    & 386/3                & 301/3                                                                        & 291/1                                                    \\ 
\hline
des\_perf                    & 0.60                                                                         & 0.6318                                                                        & 30.251               & 30.077 (-0.58\%)                                                             & 30.144 (-0.35\%)                                        & 576                  & 398 (-30.94\%)                                                                & 2322                                                    & 491/1                & 393/1                                                                        & 380/5                                                    \\ 
\hline
pci\_bridge32                & 0.75                                                                         & 0.7805                                                                        & 17.458               & 17.458 (-0.00\%)                                                             & 17.457 (-0.01\%)                                        & 92                   & 54 (-41.30\%)                                                                 & 2336                                                    & 24/1                 & 22/1                                                                         & 23/1                                                     \\ 
\hline
wb\_conmax                   & 0.79                                                                         & 0.8581                                                                        & 20.818               & 20.714 (-0.50\%)                                                             & 20.733 (-0.41\%)                                        & 290                  & 242 (-16.55\%)                                                                & 3193                                                    & 86/0                 & 78/0                                                                         & 73/0                                                     \\ 
\hline
\multicolumn{1}{|c}{Average} & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                                          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-0.27\%}                                                  & \multicolumn{1}{c}{-0.62\%}                             & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-44.54\%}                                                  & \multicolumn{1}{c}{}                                    & \multicolumn{1}{c}{} & \multicolumn{1}{c}{+3.27\%}                                                  & -7.78\%                                                  \\ 
\hline
\multicolumn{1}{|c}{Maximum} & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                                          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-0.58\%~}                                                 & \multicolumn{1}{c}{-1.84\%}                             & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-76.61\%}                                                  & \multicolumn{1}{c}{}                                    & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-22.02\%}                                                 & -31.03\%                                                 \\
\hline
\end{tabular}
}
\vspace{-2mm}
\end{table*}

==> sec/tbl-within-design.tex <==
\begin{table*}[t]
\centering
% \vspace{-6mm}
\caption{ECO timing result comparison for three different flows in area, runtime, cell change metrics}
\vspace{-4mm}
\label{tbl:within-design-10mV}
\hspace*{-2mm}
%\resizebox{1.05\linewidth}{!}{
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{Designs}     & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Target\\Delay\\(ns)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Initial\\Delay\\(ns)\end{tabular}} & \multicolumn{5}{c|}{Area($\mu$m$^2$)}                                                                                                                                                                   & \multicolumn{4}{c|}{Runtime(s)}                                                                                                                                                     & \multicolumn{3}{c|}{\# of Upsize/Downsize}                                                                                                                     \\ 
\cline{4-15}
                             &                                                                              &                                                                               & LR                   & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Inference across\\Timing Constraints\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}RL-LR\\Training\end{tabular}} & LR                   & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Inference~across \\Timing Constraints\end{tabular}} & \begin{tabular}[c]{@{}c@{}}RL-LR\\Training\end{tabular} & LR                   & \begin{tabular}[c]{@{}c@{}}Inference~across\\Timing Constraints\end{tabular} & \begin{tabular}[c]{@{}c@{}}RL-LR\\Training\end{tabular}  \\ 
\hline
des\_area                    & 0.56                                                                         & 0.5896                                                                        & 2436.3               & 2460.5               & -0.99\%                                                                    & 2424.6               & 1.24\%                                                & 113                  & 33                   & 70.80\%                                                                     & 2251                                                    & 48/1                 & 74/2                                                                         & 26/4                                                     \\ 
\hline
wb\_dma                      & 0.47                                                                         & 0.4859                                                                        & 4748.1               & 4751.3               & -0.07\%                                                                    & 4740.4               & 0.16\%                                                & 29                   & 14                   & 51.72\%                                                                     & 2285                                                    & 12/0                 & 9/0                                                                          & 8/3                                                      \\ 
\hline
pid\_controller              & 0.75                                                                         & 0.7814                                                                        & 5520.3               & 5513.9               & 0.12\%                                                                     & 5499.3               & 0.38\%                                                & 107                  & 26                   & 75.76\%                                                                     & 2718                                                    & 29/2                 & 25/4                                                                         & 26/6                                                     \\ 
\hline
aes\_cipher\_top             & 0.89                                                                         & 0.9412                                                                        & 14799.0              & 14486.0              & 2.12\%                                                                     & 14460.0              & 2.29\%                                                & 127                  & 113                  & 55.52\%                                                                     & 3015                                                    & 386/3                & 99/0                                                                         & 103/1                                                    \\ 
\hline
des\_perf                    & 0.60                                                                         & 0.6318                                                                        & 27454.0              & 27274.0              & 0.66\%                                                                     & 27183.0              & 1.19\%                                                & 354                  & 103                  & 70.79\%                                                                     & 3103                                                    & 347/1                & 230/0                                                                        & 185/1                                                    \\ 
\hline
pci\_bridge32                & 0.75                                                                         & 0.7805                                                                        & 25828.0              & 25824.0              & 0.02\%                                                                     & 25824.0              & 0.02\%                                                & 78                   & 51                   & 34.19\%                                                                     & 2794                                                    & 24/1                 & 21/1                                                                         & 24/3                                                     \\ 
\hline
wb\_conmax                   & 0.81                                                                         & 0.8581                                                                        & 22195.0              & 22130.0              & 0.29\%                                                                     & 22108.0              & 0.39\%                                                & 241                  & 125                  & 48.13\%                                                                     & 3123                                                    & 81/0                 & 55/0                                                                         & 45/2                                                     \\ 
\hline
\multicolumn{1}{|c}{Average} & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                                          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.30\%}                                                 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.81\%}                            & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{58.13\%}                                                 & \multicolumn{1}{c}{}                                    & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}                                                         &                                                          \\ 
\hline
\multicolumn{1}{|c}{Maximum} & \multicolumn{1}{c}{}                                                         & \multicolumn{1}{c}{}                                                          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{2.12\%}                                                 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{2.29\%}                            & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{75.76\%}                                                 & \multicolumn{1}{c}{}                                    & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}                                                         &                                                          \\
\hline
\end{tabular}
}
\vspace{-2mm}
\end{table*}
